Modelling Neutron Star-Black Hole Binaries: Future Pulsar Surveys and Gravitational Wave Detectors

Binaries comprised of a neutron star (NS) and a black hole (BH) have so far eluded observations as pulsars and with gravitational waves (GWs). We model the formation and evolution of these NS+BH binaries - including pulsar evolution - using the binary population synthesis code COMPAS. We predict the presence of a total of 50-2000 binaries containing a pulsar and a BH (PSR+BHs) in the Galactic field. We find the population observable by the next generation of radio telescopes, represented by the SKA and MeerKAT, current (LIGO/Virgo) and future (LISA) GW detectors. We conclude that the SKA will observe 1-80 PSR+BHs, with 0-4 binaries containing millisecond pulsars. MeerKAT is expected to observe 0-40 PSR+BH systems. Future radio detections of NS+BHs will constrain uncertain binary evolution processes such as BH natal kicks. We show that systems in which the NS formed first (NSBH) can be distinguished from those where the BH formed first (BHNS) by their pulsar and binary properties. We find 40% of the LIGO/Virgo observed NS+BHs from a Milky-Way like field population will have a chirp mass $\geq 3.0$ M$_\odot$. We estimate the spin distributions of NS+BHs with two models for the spins of BHs. The remnants of BHNS mergers will have a spin of $\sim$0.4, whilst NSBH merger remnants can have a spin of $\sim$0.6 or $\sim$0.9 depending on the model for BH spins. We estimate that approximately 25-1400 PSR+BHs will be radio alive whilst emitting GWs in the LISA frequency band, raising the possibility of joint observation by the SKA and LISA.

==> Modelling Neutron Star-Black Hole Binaries_ Future Pulsar Surveys and Gravitational Wave Detectors_v2/MeerKAT.tex <==
\begin{table}
    \caption{Estimates of the number of observed NSBHs and BHNSs from our Fiducial model under several different assumptions about our mock survey with MeerKAT. We report the number of detections relative to our default MeerKAT survey as $\mathcal{F}$, which we take to be model independent.}
    \hspace{0.5cm}
    \begin{tabular}{lcccc}
    \hline
    Telescope Survey & NSBH & BHNS & total & $\mathcal{F}$ \\
    
    \hline

MeerKAT & 5 & 10 & 15 & 1.0  \\
MeerKAT$_\mathrm{F}$ & 9 & 21 & 30 & 2.0   \\
MeerKAT$_\mathrm{T}$ & 9 & 15 & 24 & 1.6 \\
MeerKAT$_\mathrm{G}$ & 8 & 12  & 20 & 1.4 \\
MeerKAT$_\mathrm{GT}$ & 7 & 11 & 18 & 1.2  \\

 
    \hline
    \end{tabular}

    \label{tab:MeerKAT_rates}
\end{table}

==> Modelling Neutron Star-Black Hole Binaries_ Future Pulsar Surveys and Gravitational Wave Detectors_v2/NetNumbers.tex <==
\begin{table*}
\label{table:models}
    \resizebox{0.95\textwidth}{!}{\begin{minipage}{\textwidth}
    \hspace{-1.3cm}
    \begin{tabular}{ |l|rrrrr|rrrrr|rrrrcc| }
    \hline
    Model &  \multicolumn{5}{c}{NSBH}  &  \multicolumn{5}{c}{BHNS} &  total & total & DNS & DNS& $\mathcal{R}$ & $\mathcal{R}_\mathrm{SKA}$ \\
    \hline
     & net & radio & Parkes & MeerKAT & SKA & net & radio & Parkes & MeerKAT & SKA & Parkes & SKA & Parkes  & SKA & &\\
   
    \hline
Fiducial$^*$   & 764 & 145 & 3 & 5 & 9 & 27599 & 518 & 5 & 10 & 21 & 8 & 30 & 27 & 78 & 0.29  & 0.38 \\
BHK-Z$^\dagger$    & 2231 & 299 & 18 & 23 & 50 & 123090  & 1747 & 22 & 33 & 72 & 40 & 122 & 27  & 71 & 1.48  & 1.72 \\

BHK-F$^*$    & 297 & 62 & 2 & 3 & 7 & 5074 & 60 & 1 & 1 & 2 & 3 & 9 & 25  & 72 & 0.12 & 0.13 \\
CE-P$^*$    & 36 & 1 & 0 & 0 & 0 & 23541 & 185 & 2 & 4 & 6 & 2 & 6 & 21  & 62 &0.10 & 0.10 \\
CE-Z$^\dagger$    & 734 & 7 & 0 & 0 & 0 & 27325 & 483 & 5 & 9 & 18 & 5 & 18 & 3  & 11 &1.67 & 1.64 \\
ZM-001$^*$    & 7754 & 103 & 1 & 1 & 3 & 45867 & 533 & 8 & 10 & 21 & 9 & 24 &  14 & 45 &0.64 & 0.53 \\
ZM-02$^*$    & 467 & 66 & 2 & 3 & 6 & 12895 & 120 & 2 & 2 & 4 & 4 & 10 & 40 & 121 &0.10 & 0.08 \\
FDT-500$^*$    & 823 & 94 & 3 & 3 & 6 & 26631 & 461 & 5 & 8 & 18  & 8 & 24 &  20 & 62 & 0.40 & 0.39 \\
FDM-20$^*$    & 902 & 93  & 3 & 4 & 9 & 27807 & 500 & 5 & 10 & 20 & 7 & 29 & 19  & 64 &0.37 &0.45 \\
BMF-FL$^\dagger$    & 7900 & 2939 & 90 & 125 & 264 & 275782 & 32421 & 551 & 877 & 1910 & 641 & 2174 & 78 & 239 &8.21 &9.10 \\
RM-R$^*$ & 480 & 26 & 0 & 0 & 0 & 77141 & 975 & 11 & 19 & 40 & 11 & 40 & 33 & 85 & 0.33 & 0.47\\

    \hline
    \end{tabular}
    \end{minipage}
    }
    \caption{Quantitative distributions of NS+BHs for each model scaled to a population representative of the Milky Way. The column `net' signifies the total count of binaries: both radio and non-radio. The survey observed data-sets are hence a subset to the radio population, after accounting for the radio observational biases. The column `total' signifies the combined survey-observed NSBH and BHNS systems, post-radio-selection effects.
    The ratio of the number of observations by Parkes, estimating the current detection rate of NS+BH per DNS is given by $\mathcal{R}$ = (Parkes: NS+BH)/(Parkes: DNS). To estimate the future detection rate we quote $\mathcal{R}_\mathrm{SKA}$ = (SKA: NS+BH)/(SKA: DNS).
    Superscripts $*$ and $\dagger$
    on model names denote feasible or unfeasible models respectively on the basis of order of magnitude disparity in detection rates. The Poisson uncertainty for $\mathcal{R}$ and $\mathcal{R}_\mathrm{SKA}$ remain $\lessapprox$0.2 for all models.}
    \label{tab:netNumbers}
\end{table*}

==> Modelling Neutron Star-Black Hole Binaries_ Future Pulsar Surveys and Gravitational Wave Detectors_v2/ZAMS.tex <==
\begin{table*}
\begin{tabular}{lrrrrrrrr}
\hline 
Variable    & M$_\mathrm{NS}$ (ZAMS) & M$_\mathrm{BH}$ (ZAMS) & M$_\mathrm{NS}$ & M$_\mathrm{BH}$ & a (ZAMS) & a(DCO) & t$_\mathrm{birth}$ & $\Delta$t$_\mathrm{form}$ \\
            & $\mathrm{M_\odot}$             & $\mathrm{M_\odot}$             & $\mathrm{M_\odot}$      & $\mathrm{M_\odot}$      & AU      & AU & Gyrs   & Myrs              \\
            \hline
BHNS\_total   &      20.82            &    59.24              &    1.45       &   6.78        &    4.77     &  2.81  &   7.97     &      13.41             \\
BHNS\_radio &     37.93             &       69.35           &    1.50       &     7.88      &     3.34    &  0.94  &   12.78     &         9.38          \\
NSBH\_total   &     23.26             &        18.01          &     1.48      &    3.85       &    0.67     & 0.22   &   7.16     &      11.86             \\
NSBH\_radio &       23.01           &     17.00             &    1.49       &  3.42  &0.39       &   0.07      &  10.87  &    12.40    \\                
\hline
\end{tabular}
\caption{Mean values of binary parameters for NS+BH binaries in our Fiducial model. While "(ZAMS)" refers to the parameter mean value at zero-age  at sequence, "(DCO)" refers to the same at the formation of the double compact object. t$_\mathrm{birth}$ denotes the birth time of the pulsar (in a 13 Gyr old Milky Way) while $\Delta$t$_\mathrm{form}$ signifies the time taken by the binary to evolve from zero-age main sequence star to double compact object. The distributions of some these quantities are shown in Section~\ref{sec:results_radio}.}
\label{tab:ZAMS_radioVSnet}
\end{table*}

==> Modelling Neutron Star-Black Hole Binaries_ Future Pulsar Surveys and Gravitational Wave Detectors_v2/meanValuesSKA.tex <==

 \begin{table*}
 \label{table:models}
 \resizebox{0.8\textwidth}{!}{
 
 \begin{minipage}[l]{\textwidth}
 \hspace{-2cm}
 \begin{tabular}{|l|rrrrrrrr|rrrrrrrr}
 \hline
 Model &  \multicolumn{8}{c|} {NSBH}  &  \multicolumn{8}{c|}{BHNS}  \\
 \hline
 & $P$ & $\Dot{P}$ & $B$ & $P_{\mathrm{orb}}$ & $e$ & $m_{\mathrm{psr}}$ & $m_{\mathrm{cmp}}$ & $|Z|$ & $P$ & $\Dot{P}$ & $B$ & $P_{\mathrm{orb}}$ & $e$ & $m_{\mathrm{psr}}$ & $m_\mathrm{{cmp}}$ & $|Z|$  \\
 & s & s/s & Gauss & days & - & M$_\odot$ & M$_\odot$ & Kpc & s & s/s & Gauss & days & - & M$_\odot$ & M$_\odot$ & Kpc \\
   
 \hline
Fiducial   & 0.047 & 1.952e-17 & 1.626e10 & 25.836 & 0.777 & 1.504 & 3.284 & 0.807 & 1.058 & 8.555e-15 & 1.217e12 & 80.252 & 0.262 & 1.504 & 7.688 & 0.186\\

BHK-Z & 0.025 & 9.699e-18 & 6.923e09 & 88.373 & 0.890 & 1.513 & 3.244 & 0.222 & 0.983 & 4.246e-15 & 1.102e12 & 136.315 & 0.274 & 1.505 & 5.699 & 0.209\\
BHK-F   & 0.028 & 9.560e-19 & 4.648e09 & 46.515 &  0.888 & 1.508 & 3.797 & 1.813 & 1.113 & 2.672e-15 & 1.160e12 & 604.350 & 0.322 & 1.427 & 5.963 & 0.245\\


CE-P   & 0.239 & 1.298e-16 & 1.039e11 & 5.017 &  0.304 & 2.067 & 5.276 & 0.324 & 0.866 & 3.616e-15 & 9.452e11 & 673.042 & 0.419 & 1.495 & 6.3933 & 0.232\\
CE-Z   & 0.823 & 9.082e-16 & 6.722e07 & 78.275 & 0.558 & 1.564  & 4.121  &  0.294 & 1.129 &  5.806e-15  & 1.275e12 & 1550.569 & 0.246 & 1.516 & 7.968 &  0.198\\

ZM-001   & 0.659 & 1.255e-15 & 6.689e11 & 4.884  & 0.431 & 1.605 & 14.653 & 0.213 & 0.954 & 1.311e-14 & 1.229e12 & 14093.453 & 0.421 & 1.741 & 10.678 & 0.262\\
ZM-02   & 0.045 & 5.165e-18 & 8.182e09 & 18.032 & 0.758 & 1.455 & 2.989 & 0.581 & 0.972 & 2.815e-15 & 1.024e12 & 1368.329 & 0.400 & 1.415 & 5.340 & 0.181\\

FDT-500   & 0.033 & 2.500e-17 & 1.485e10 & 1346.088 & 0.796 & 1.522 & 3.328 & 1.108 & 1.055 & 4.200e-15 & 1.204e12 & 142.553 & 0.235 & 1.491 & 7.863 & 0.172 \\
FDM-20   & 0.126 & 1.079e-17 & 2.217e10 & 3.887 & 0.637 & 1.518 & 3.411 & 0.467 & 1.101 & 2.793e-14  & 1.209e12 & 736.782 &  0.255 & 1.516 & 7.919 & 0.214\\
BMF-FL   & 0.022 & 3.423e-18 & 4.918e09 & 6311.351  & 0.813 & 1.558 & 3.256 &  0.855 & 0.323 & 1.985e-16 & 1.243e11 & 1276.610 &  0.359 & 1.485 & 7.131 & 0.233\\

RM-R & 0.448 & 2.243e-16 & 2.237e-11 & 1201.290 & 0.293 & 1.309 & 7.490 & 0.171 & 1.079 & 8.380e-15 & 1.115e-12 & 393.102 & 0.253 & 1.242 & 7.950 & 0.246\\
    \hline
    \end{tabular}
    
    \end{minipage}}
    \caption{Mean values of radio observables for PSR+BH binaries observed by the SKA. This population accounts for radio selection effects as described in Section~\ref{subsec:radio_selection_effects}. We show the values for both NSBHs and BHNSs for each of our models.}
    \label{tab:radioObservablesMean:SKA}
  \end{table*}


==> Modelling Neutron Star-Black Hole Binaries_ Future Pulsar Surveys and Gravitational Wave Detectors_v2/meanValues_Observables.tex <==
\begin{table*}
\label{table:models}
    \resizebox{0.8\textwidth}{!}{\begin{minipage}{\textwidth}
    \hspace{-2cm}
    \begin{tabular}{|l|rrrrrrrr|rrrrrrrr}
    \hline
    Model &  \multicolumn{8}{c|} {NSBH}  &  \multicolumn{8}{c|}{BHNS}  \\
    \hline
     & $P$ & $\Dot{P}$ & $B$ & $P_{\mathrm{orb}}$ & $e$ & $m_{\mathrm{psr}}$ & $m_{\mathrm{cmp}}$ & $|Z|$ & $P$ & $\Dot{P}$ & $B$ & $P_{\mathrm{orb}}$ & $e$ & $m_{\mathrm{psr}}$ & $m_\mathrm{{cmp}}$ & $|Z|$  \\
     & s & s/s & Gauss & days & - & M$_\odot$ & M$_\odot$ & Kpc & s & s/s & Gauss & days & - & M$_\odot$ & M$_\odot$ & Kpc \\
   
    \hline
Fiducial   & 0.104 & 5.992e-17 & 5.424e10 & 10.702 & 0.511 & 1.491 & 3.417 &  0.385 & 3.135 & 5.420e-15 & 2.074e12 & 239.922 & 0.231  & 1.496 & 7.884 &  0.160\\
BHK-Z   & 0.079  & 4.358e-17 & 3.535e10 & 1473.933 & 0.882 & 1.516 & 3.272 & 0.134 & 3.112 & 5.596e-15  &2.029e12 & 178.434  & 0.250 & 1.474 & 5.747 & 0.227\\
BHK-F   &  0.081 & 1.012e-17 & 2.424e10 & 20.174 & 0.645 & 1.504 & 3.615 & 2.086 & 3.272 & 3.458e-15 & 2.002e12 & 904.641 & 0.305 & 1.427 & 6.025 &  0.194 \\
CE-P   & 0.925 & 4.956e-16 & 5.128e11 & 160.451 & 0.473 & 2.014 & 4.897 & 0.595 &2.946  &  3.559e-15 & 1.915e12 & 16653.155 & 0.389 & 1.493 & 6.474 & 0.215\\
CE-Z   & 2.465 & 1.471e-15 & 1.448e12 & 82.078 &  0.552 & 1.544  & 4.060 & 0.561 & 3.272 & 4.863e-15 & 2.149e12 & 1110.678 & 0.232 & 1.500 & 7.995 & 0.177 \\
ZM-001   & 1.673 & 1.384e-15 & 1.087e12 & 5.470 & 0.353 & 1.807 &  14.486 & 0.164 & 2.996 & 6.970e-15 & 2.175e12 & 9515.507 & 0.394 & 1.749 & 10.663 &  0.238 \\
ZM-02   & 0.120 & 3.361e-17 &  5.482e10 & 8.856 & 0.479 & 1.438 & 3.041 & 0.575 & 3.316 & 6.182e-15 & 2.070e12 & 490.496 & 0.367 & 1.365 & 5.027 & 0.175\\
FDT-500   & 0.061 & 2.450e-17 & 2.861e10 & 856.467 & 0.544 & 1.514 & 3.314 & 0.600 & 3.124  & 3.480e-15 & 2.090e12 & 214.027 & 0.228 & 1.491 & 7.951 & 0.164\\
FDM-20   & 0.191 & 4.420e-17  & 6.018e10 & 3.409 & 0.544 & 1.527 & 3.371 & 0.445 &  3.211 & 8.718e-15 & 2.150e12 & 445.976 & 0.237 & 1.502 & 7.936 & 0.169\\
BMF-FL   & 0.038 & 5.864e-18 & 9.134e09 & 2452.445 & 0.582 & 1.520 & 3.345 & 0.553 & 0.519 & 2.095e-16 &  1.849e11 & 847.694 & 0.255 & 1.460 & 7.592 & 0.179\\

RM-R & 0.334 & 1.335-16 & 1.475e-11 & 832.403 & 0.108 & 1.249 & 7.598 & 0.112 & 3.242 & 5.416e-15 & 1.953e-12 & 759.672 & 0.231 & 1.234 & 7.978 & 0.226\\
    \hline
    \end{tabular}
    \end{minipage}}
    \caption{Mean values of radio observables for PSR+BH binaries. We show the values for both NSBH and BHNS sub-populations for each of our models.}
    \label{tab:radioObservablesMean:Radio}
\end{table*}

==> Modelling Neutron Star-Black Hole Binaries_ Future Pulsar Surveys and Gravitational Wave Detectors_v2/modelsTable.tex <==
% \begin{table*}

\begin{table*}
    \resizebox{0.85\textwidth}{!}{\begin{minipage}{\textwidth}
    \hspace{-1.9cm}
    \begin{tabular}{lrrrrrrrrrr}
    \hline
    Model & Mass Range & BH kick prescription & CE model & CE accretion &$\tau_d$ & $\Delta M_d$ & $B_\mathrm{birth}$ distribution & $B_\mathrm{spin}$ distribution & Metallicity & Supernovae Prescription\\
    & ($\mathrm{M_\odot}$) & - & - & - &(Myrs) & ($\mathrm{M_\odot}$) & - & - & (Z) & - \\
    \hline
Fiducial   & 4--100 & Fallback & Optimistic& Macleod+ &1000 & 0.15 & Uniform & Uniform & 0.0142  & Delayed\\
BHK-Z   & 4--100 & Zero & Optimistic & Macleod+ &1000 & 0.15 & Uniform & Uniform & 0.0142 & Delayed\\
BHK-F   & 4--100 & Full & Optimistic &  Macleod+& 1000 & 0.15 & Uniform & Uniform & 0.0142 & Delayed \\ 
CE-P   & 4--100 & Fallback & Pessimistic & Macleod+ &1000 & 0.15 & Uniform & Uniform & 0.0142 & Delayed \\
CE-Z & 4-100 & Fallback & Optimistic & Zero& 1000 & 0.15 & Uniform & Normal &0.0142  & Delayed \\
ZM-001 & 4--100 & Fallback & Optimistic & Macleod+ & 1000 & 0.15 & Uniform & Uniform & 0.001  & Delayed\\
ZM-02 & 4--100 & Fallback & Optimistic & Macleod+ & 1000 & 0.15 & Uniform & Uniform & 0.02  & Delayed\\
FDT-500  & 4--100 & Fallback & Optimistic & Macleod+ & 500 & 0.15 & Uniform & Uniform & 0.0142  & Delayed\\  
FDM-20 & 4--100 & Fallback & Optimistic & Macleod+ & 1000 & 0.2 & Uniform & Uniform & 0.0142 & Delayed \\  
BMF-FL & 4--100 & Fallback & Optimistic & Macleod+ & 1000 & 0.15 & Flat in Log & Uniform & 0.0142  & Delayed\\
RM-R   & 4--100 & Fallback & Optimistic& Macleod+ &1000 & 0.15 & Uniform & Uniform & 0.0142 & Rapid \\



    \hline
    \end{tabular}
    \end{minipage}}
    \caption{Suite of models used for the analysis. Each model following Fiducial has one parameter that has been varied from it.} 
    \label{tab:NSBH}
\end{table*}


==> Modelling Neutron Star-Black Hole Binaries_ Future Pulsar Surveys and Gravitational Wave Detectors_v2/radioLifetime.tex <==
\begin{table}
    \begin{tabular}{lrrrrr}
    \hline
    Model  & \multicolumn{3}{c}{$r_\mathrm{birth}$ (Myrs$^{-1}$)} &  \multicolumn{2}{c}{$t_\mathrm{radio}$ (Myrs)}  \\
    &&&&&\\
     & NSBH & BHNS & NS+BH & NSBH & BHNS \\
    % &   $t_\mathrm{radiolife}$& $t_\mathrm{radiolife}$\\
    \hline
     Fiducial & 0.10 & 8.31 & 8.41 &1333 & 65\\
     BHK-Z & 0.13 & 27.74 & 27.87 &847 & 67 \\
     BHK-F & 0.05 & 1.05 & 1.10 &1197 & 64\\
     CE-P & 0.003 & 2.67 & 2.67 &137 & 74\\
     CE-Z & 0.08 & 8.23 & 8.31 &77 & 63 \\
     ZM-001 & 1.49 & 8.56 & 10.05 &87 & 72\\
     ZM-02 & 0.05 & 2.08 & 2.13 &1351 & 71\\
     FDT-500 & 0.09 & 8.04 & 8.13 & 873 & 59\\
     FDM-20 & 0.11 & 8.27& 8.38 &919 & 65\\
     BMF-FL & 0.10 & 8.15 & 8.25 &3252 & 435 \\
     RM-R  & 0.07 & 16.94 & 17.01 &476 &  63 \\
    \hline
    \end{tabular}
    \caption{Average birth rates $r_\mathrm{birth}$ and radio lifetimes $t_\mathrm{radio}$ of NSBH and BHNS binaries in each of our models. 
    In general, pulsars in BHNSs are non-recycled and have shorter lifetimes than the partially recycled pulsars in NSBHs.
    The birth rates $r_\mathrm{birth}$ are a function of the binary evolution parameters rather than the pulsar ones. 
    Hence the Fiducial model, FDT-500, FDM-20 and BMF-FL all have similar ranges of birth rates.
    }
    \label{table:radio_lifetime}
\end{table}

==> Modelling Neutron Star-Black Hole Binaries_ Future Pulsar Surveys and Gravitational Wave Detectors_v2/telescope_specs.tex <==
\begin{table}
    \caption{Telescope specifications assumed in this work, based on (a) Parkes Multibeam Survey \citep{Manchester:2001}, (b) TRansients and PUlsars with MeerKAT (TRAPUM), MeerKAT Large Survey Projects \citep{Stappers:2018Le}, (c) Square Kilometer Array Pulsar Search \citep{Grainge:2017,Levin:2017mkq}. We assume a central observing frequency of 1400\,MHz for all surveys. Columns $T_\mathrm{rec}$, $t_\mathrm{samp}$ and $t_\mathrm{int}$ signify receiver temperature, sampling time and integration time respectively.}
    \hspace{-1.0cm}
    \begin{tabular}{lrrrrrr}
    \hline
    Telescope & Bandwidth & Gain & $T_\mathrm{rec}$ & $t_\mathrm{samp}$ & $t_\mathrm{int}$ & Coverage \\
    survey & (MHz) &  & (K) & ($\mu$s) & (s) & - \\
    \hline

Parkes$^{(a)}$  & 288 & 0.65 & 24 & 256 & 2100 & all-sky\tablefootnote{We do not apply a cut-off to the sky coverage of our Parkes-like survey, since we are using it as a representative proxy for the multiple surveys that have discovered DNSs across the globe.
} \\
MeerKAT$^{(b)}$ & 400 & 1.80 & 18 & 64 & 637 & Galactic-plane\tablefootnote{cut-off point:$|b|<5.2$ and $-110^{\circ}<l<10^{\circ}$}   \\
MeerKAT$_\mathrm{F}$ & 800 & 2.80 & 18 & 64 & 2100 & all-sky-cutoff\tablefootnote{cut-off point: $\delta<30^{\circ} $}  \\
MeerKAT$_\mathrm{T}$ & 800 & 2.80 & 18 & 64 & 300 & all-sky-cutoff$^{3}$  \\
MeerKAT$_\mathrm{G}$ & 800 & 2.80 & 18 & 64 & 2100 & Galactic-plane\tablefootnote{cut-off point:  $-5^{\circ}<\delta<5^{\circ}$}  \\
MeerKAT$_\mathrm{GT}$ & 800 & 2.80 & 18 & 64 & 300 & Galactic-plane$^{4}$  \\
SKA$^{(c)}$     & 300 & 8.40 & 30 & 64 & 2100 & all-sky-cutoff$^{3}$ \\
    \hline
    \end{tabular}
    \label{table:telescope_specs}
\end{table}
